StarDist: A Code Generator for Distributed Graph Algorithms

We introduce StarDist, a Domain Specific Language for generating high-performant distributed graph algorithms in the message passing model. Our analysis-transformation framework optimizes graph traversal based on graph property access patterns, reduces global lock acquisitions on distributed structures, and minimizes message queues used in reduction operations. We provide a network optimized communication runtime for reduction operations that couples with our analysis framework and optimizes the propagation of updates based on vertex residency. StarDist is able to identify monotonic reduction blocks and is able to fuse reduction iterations over graphs into \textit{pulses}. We evaluate StarDist using three fundamental graph algorithms belonging to the CONGEST model: single-source shortest paths, weakly connected components, and PageRank computation, using a suite comprising both real-world and synthetic graphs across varying densities of topological compaction. Our results illustrate that the code generated with StarDist outperforms the distributed frameworks DRONE and D-Galois by an average of 19$\times$ and 7$\times$, respectively on our high communication setup and by 1.4$\times$ and 1.92$\times$ respectively on our high congestion network setup when averaged across all three algorithms.

==> Experiments/comparison_60_sssp/comp60rd.tex <==
graph               np  
GM                  60  16.84    388.324 11.108      47.244       29.256 10.966 157.813768
US                  60  120.19   2000     2000       2000         357.425 1645.312 2000 


==> Experiments/strong_scale_wcc/fused/germ.tex <==
nprocs  time
10  19.560871
20  12.018099
30  10.124021
40  15.726507
50  17.753249
60  21.332270
70  24.898832
80  30.940434
90  33.170496

==> Experiments/strong_scale_wcc/fused/liv.tex <==
nprocs time
10  17.115325
20  13.531467
30  10.557626
40  8.688209
50  7.259597
60  8.046739
70  6.355263
80  6.120485
90  6.096582


==> Experiments/strong_scale_wcc/fused/orkut.tex <==
nprocs time
10  44.088512
20  32.956698
30  25.045406
40  21.865286
50  22.024579
60  18.294438
70  14.176955
80  14.028904
90  14.063038

==> Experiments/strong_scale_wcc/fused/pok.tex <==
nprocs  time
10  12.507844
20  7.995435
30  6.330626
40  4.680299
50  4.041973
60  3.364793
70  2.975778
80  2.612956
90  2.397750

==> Experiments/strong_scale_wcc/fused/rmat.tex <==
nprocs time
10  41.588312
20  38.659983
30  37.240757
40  32.733409
50  30.845674
60  26.195236
70  27.166411
80  28.216908
90  25.235988

==> Experiments/strong_scale_wcc/fused/u10.tex <==
nprocs time
10  77.788489
20  42.358483
30  27.549664
40  22.475994
50  17.468967
60  14.398398
70  12.380630
80  12.459952
90  11.213158

==> Experiments/strong_scale_wcc/fused/usa.tex <==
nprocs time
10  249.657064
20  190.803269
30  166.731754
40  148.132238
50  148.629834
60  137.839594
70  142.207740
80  130.383856
90  141.902437

==> Experiments/strong_scale_wcc/fused/wiki.tex <==
nprocs  time
10  24.604436
20  17.544905
30  14.231725
40  12.442897
50  12.255528
60  9.868854
70  10.974827
80  9.120479
90  7.827149

==> Experiments/strong_scale_wcc/nonfused/germ.tex <==
nprocs time
10	18.760243
20	11.56676
30	9.770928
40	15.918277
50	18.004378
60	20.975994
70	24.174716
80	27.556409
90	31.017223

==> Experiments/strong_scale_wcc/nonfused/liv.tex <==
nprocs time
10	18.589956
20	14.317033
30	11.488463
40	9.17308
50	7.716033
60	8.621217
70	6.856045
80	6.368107
90	6.515559

==> Experiments/strong_scale_wcc/nonfused/orkut.tex <==
nprocs time
10	46.730687
20	33.399379
30	25.7558
40	22.339538
50	22.467844
60	18.790978
70	14.534001
80	15.216935
90	15.91095

==> Experiments/strong_scale_wcc/nonfused/pok.tex <==
nprocs	time
10	13.433791
20	8.505167
30	6.680721
40	4.976021
50	4.23356
60	3.555682
70	3.064178
80	2.698319
90	2.481453

==> Experiments/strong_scale_wcc/nonfused/rmat.tex <==
nprocs time
10	44.510787
20	41.249075
30	38.548433
40	35.074315
50	32.71699
60	26.993023
70	28.125779
80	29.488333
90	25.576539

==> Experiments/strong_scale_wcc/nonfused/u10.tex <==
nprocs time
10	88.544818
20	47.108904
30	30.961216
40	25.771992
50	20.007296
60	16.561049
70	14.067461
80	13.712009
90	12.313845

==> Experiments/strong_scale_wcc/nonfused/usa.tex <==
nprocs time
10	255.712932
20	195.674607
30	170.34541
40	150.72207
50	151.049122
60	140.219471
70	142.785139
80	131.384309
90	141.441253

==> Experiments/strong_scale_wcc/nonfused/wiki.tex <==
nprocs time
10	27.229982
20	18.432437
30	15.012336
40	12.79686
50	12.795548
60	10.866734
70	11.710014
80	9.717696
90	8.405076
